A time-frequency approach to relativistic correlations in quantum field theory

Moving detectors in relativistic quantum field theories reveal the fundamental entangled structure of the vacuum which manifests, for instance, through its thermal character when probed by a uniformly accelerated detector. In this paper, we propose a general formalism inspired both from signal processing and correlation functions of quantum optics to analyze the response of point-like detectors following a generic, non-stationary trajectory. In this context, the Wigner representation of the first-order correlation of the quantum field is a natural time-frequency tool to understand single-detection events. This framework offers a synthetic perspective on the problem of detection in relativistic theory and allows us to analyze various non-stationary situations (adiabatic, periodic) and how excitations and superpositions are deformed by motion. It opens up interesting perspective on the issue of the definition of particles.

==> tikz/acc_startstop_obs.tex <==
\begin{tikzpicture}
%\input{tikz/styles/dot.tex}
\tikzstyle{dot}=[draw,circle,minimum size=2pt,inner sep=0pt,
	outer sep=0pt,fill]
\tikzset{%
    add/.style args={#1 and #2}{
        to path={%
 ($(\tikztostart)!-#1!(\tikztotarget)$)--($(\tikztotarget)!-#2!(\tikztostart)$)%
  \tikztonodes},add/.default={.2 and .2}}
}  


\def\le{3}
\def\lengthcone{2}


%%%%%%%
%Vrai tracé
%%%%%%%

\begin{scope}[shift={(0,0)}]
	\draw[->] (0,-0.8*\le) -- (0,0.8*\le) node[anchor=west] {$ct$};
	\draw[->] (-0.3*\le,0) -- (0.9*\le,0) node[anchor=west] {$x$};
	
		
	\def\posobs{65}
	\def\posi{53}
	\pgfmathsetmacro\posf{2*\posobs-\posi}
	\def\startmark{0.02}
	\def\endmark{0.94}
	\def\step{0.01}
	\pgfmathsetmacro\numcones{min(\posobs,floor((\endmark-\startmark)/\step)-\posobs)}	
	
	%On nomme les points réguliers le long de la courbe de Béziers
	\pgfmathsetmacro{\a}{1.5}
	\pgfmathsetmacro{\tau}{0.3}
	\pgfmathsetmacro{\tmax}{(2-1/\a*sinh(\a*\tau))/cosh(\a*\tau)+\tau}
		
	%On trace la ligne d'univers
	\draw[thick] 
		({1/\a*cosh(\a*\tau)-sinh(\a*\tau)*(-\tmax+\tau)},
		{-1/\a*sinh(\a*\tau)+cosh(\a*\tau)*(-\tmax+\tau)})
		--
		({1/\a*cosh(\a*\tau)},
		{-1/\a*sinh(\a*\tau)});
	\draw[thick,red]
		plot[domain=-\tau:\tau] ({1/\a*cosh(\a*\x)},{1/\a*sinh(\a*\x)});
	\draw[thick]
		({1/\a*cosh(\a*\tau)},
		{1/\a*sinh(\a*\tau)})
		--
		({1/\a*cosh(\a*\tau)+sinh(\a*\tau)*(\tmax-\tau)},
		{1/\a*sinh(\a*\tau)+cosh(\a*\tau)*(\tmax-\tau)});
	
	%On trace le cône
	\draw[dashed] (2,-2) -- (-0.3*\le,0.3*\le);
	\draw[dashed] (-0.3*\le,-0.3*\le)-- (2,2);
	
%	\draw[stealth-stealth,red] (0,-0.2) -- (1/\a,-0.2) node[midway,below]{$\frac{c^2}{a}$};
	
\end{scope}


\end{tikzpicture}


==> tikz/accelerated_observer.tex <==
\begin{tikzpicture}
%\input{tikz/styles/dot.tex}
\tikzstyle{dot}=[draw,circle,minimum size=2pt,inner sep=0pt,
	outer sep=0pt,fill]
\tikzset{%
    add/.style args={#1 and #2}{
        to path={%
 ($(\tikztostart)!-#1!(\tikztotarget)$)--($(\tikztotarget)!-#2!(\tikztostart)$)%
  \tikztonodes},add/.default={.2 and .2}}
}  


\def\le{3}
\def\lengthcone{2}


%%%%%%%
%Vrai tracé
%%%%%%%

\begin{scope}[shift={(0,0)}]
	\draw[->] (0,-0.8*\le) -- (0,0.8*\le) node[anchor=west] {$ct$};
	\draw[->] (-0.3*\le,0) -- (0.9*\le,0) node[anchor=west] {$x$};
	
		
	\def\posobs{65}
	\def\posi{53}
	\pgfmathsetmacro\posf{2*\posobs-\posi}
	\def\startmark{0.02}
	\def\endmark{0.94}
	\def\step{0.01}
	\pgfmathsetmacro\numcones{min(\posobs,floor((\endmark-\startmark)/\step)-\posobs)}	
	
	%On nomme les points réguliers le long de la courbe de Béziers
	\pgfmathsetmacro{\a}{1.5}
    \path[decoration={
		markings,
		mark=between positions \startmark and \endmark step \step with 
		\coordinate (mark-\pgfkeysvalueof{/pgf/decoration/mark info/sequence number});},
		postaction={decorate}] 
		plot[domain=-1.2:1.2] ({1/\a*cosh(\a*\x)},{1/\a*sinh(\a*\x)});
		
	%On trace la ligne d'univers
	\draw[thick,-stealth] 
		plot[domain=-1.2:1.2] ({1/\a*cosh(\a*\x)},{1/\a*sinh(\a*\x)})
		node[anchor=west] {$\mathcal{L}_{\theta}$} ;
	%On met quelques points spécifiques
	\coordinate[dot] () at (mark-\posobs);
	\node[right] at (mark-\posobs) {$O(\tau')$};
	\coordinate[dot] () at (mark-\posi);
	\node[right] at (mark-\posi) {$O(\tau)$};
	
	%On trace les surfaces de simultanéité avec ce qu'on sait analytiquement
	\draw[densely dotted, blue] [add=0 and 1] (0,0) to (mark-\posobs)
	 node[right] {$S_{O(\tau')}$};
%	\draw[densely dotted, blue] [add=0 and 2] (0,0) to (mark-\posi)
%	 node[right] {$S_{O(\tau)}$};
	 
	%On trace le cône
	\draw[dashed] (2,-2) -- (0,0);
	\path[fill, gray, opacity = 0.2] (-0.3*\le,2) --(2,2) -- (-0.3*\le,-0.3*\le) -- cycle;
	\draw[dashed] (-0.3*\le,-0.3*\le)-- (2,2) node[above,align = left, text width = 2cm]{Horizon};
	
%	\draw[stealth-stealth,red] (0,-0.2) -- (1/\a,-0.2) node[midway,below]{$\frac{c^2}{a}$};
	
\end{scope}


\end{tikzpicture}

==> tikz/beamed_accelerated_observer.tex <==
\begin{tikzpicture}
%\input{tikz/styles/dot.tex}
\tikzstyle{dot}=[draw,circle,minimum size=2pt,inner sep=0pt,
	outer sep=0pt,fill]
\tikzset{%
    add/.style args={#1 and #2}{
        to path={%
 ($(\tikztostart)!-#1!(\tikztotarget)$)--($(\tikztotarget)!-#2!(\tikztostart)$)%
  \tikztonodes},add/.default={.2 and .2}}
}  


\def\le{3}
\def\lengthcone{2}


%%%%%%%
%Vrai tracé
%%%%%%%

\begin{scope}[shift={(0,0)}]
	\pgfmathsetmacro{\pwidth}{0.3}
	\fill[red!80,opacity=0.5] (-0.3*\le, -0.3*\le-\pwidth) -- (2+\pwidth, 2)
		-- (2-\pwidth, 2) -- (-0.3*\le, -0.3*\le + \pwidth) -- cycle;
	\fill[blue!80,opacity=0.5] (2, -\pwidth) -- (2, \pwidth)
		-- (\pwidth,2) -- (-\pwidth, 2) -- cycle;
	\draw[->] (0,-0.8*\le) -- (0,0.8*\le) node[anchor=west] {$ct$};
	\draw[->] (-0.3*\le,0) -- (0.9*\le,0) node[anchor=west] {$x$};
	
		
	\def\posobs{65}
	\def\posi{53}
	\pgfmathsetmacro\posf{2*\posobs-\posi}
	\def\startmark{0.02}
	\def\endmark{0.94}
	\def\step{0.01}
	\pgfmathsetmacro\numcones{min(\posobs,floor((\endmark-\startmark)/\step)-\posobs)}	
	
	%On nomme les points réguliers le long de la courbe de Béziers
	\pgfmathsetmacro{\a}{1.5}
    \path[decoration={
		markings,
		mark=between positions \startmark and \endmark step \step with 
		\coordinate (mark-\pgfkeysvalueof{/pgf/decoration/mark info/sequence number});},
		postaction={decorate}] 
		plot[domain=-1.2:1.2] ({1/\a*cosh(\a*\x)},{1/\a*sinh(\a*\x)});
		
	%On trace la ligne d'univers
	\draw[thick,-stealth] 
		plot[domain=-1.2:1.2] ({1/\a*cosh(\a*\x)},{1/\a*sinh(\a*\x)});
	
	%On trace le cône
	\draw[dashed] (2,-2) -- (0,0);
	\path[fill, gray, opacity = 0.2] (-0.3*\le,2) --(2,2) -- (-0.3*\le,-0.3*\le) -- cycle;
	\draw[dashed] (-0.3*\le,-0.3*\le)-- (2,2) node[above,align = left, text width = 2cm]{Horizon};
	
%	\draw[stealth-stealth,red] (0,-0.2) -- (1/\a,-0.2) node[midway,below]{$\frac{c^2}{a}$};
	
\end{scope}


\end{tikzpicture}


==> tikz/different-obs.tex <==
\begin{tikzpicture}[every node/.style={font=\footnotesize},unsure/.style={green!70!black}]
	\def\leftcol{-3}
	\def\rightcol{3}
	\def\rowi{-2.5}
	\pgfmathsetmacro{\rowii}{\rowi-2}
	\pgfmathsetmacro{\rowiii}{\rowii+\rowi}
	\node (coh-xt-1) at (\leftcol,0)
		{$G^{(n)}_{\mathcal{O}}(x_1^{\mathcal{O}}, \dots, x_n^{\mathcal{O}})$};
	\node (coh-xt-2) at (\rightcol,0)
		{$G^{(n)}_{\mathcal{O'}}(x_1^{\mathcal{O'}}, \dots, x_n^{\mathcal{O'}})$};
	\node (coh-t) at (0, \rowi)
		{$G^{(n)}_{\mathcal{O} \mathcal{O'}}(\tau_1, \dots, \tau_n)$};
	\node (field-t) at (0, \rowii)
		{$\varphi_{\mathcal{O} \mathcal{O'}}(\tau)$};
	\node (field-xt-1) at (\leftcol, \rowiii)
		{$(\varphi_{\mathcal{O}}, \mathcal{H}_{\mathcal{O}}, f_{\mathcal{O}})$};
	\node (field-xt-2) at (\rightcol, \rowiii)
		{$(\varphi_{\mathcal{O'}}, \mathcal{H}_{\mathcal{O'}}, f_{\mathcal{O'}})$};
	
	\begin{scope}[every node/.style={font=\scriptsize}]
		\draw[stealth-stealth] (field-xt-1) -- (coh-xt-1)
			node[midway,above,rotate=90] {Reconstruction};
		\draw[stealth-stealth] (field-xt-2) -- (coh-xt-2)
			node[midway,above,rotate=-90] {Reconstruction};
		\draw[stealth-stealth] (field-xt-1) -- (field-xt-2)
			node[midway,below] {Bogoliubov};
		\draw[stealth-stealth] (coh-xt-1) -- (coh-xt-2)
			node[midway,above] {Covariance};
		\draw[-stealth] (coh-xt-1.330) -- (coh-t.160)
			node[midway,sloped,below] {Trajectory};
		\draw[stealth-,unsure] (coh-xt-1.340) -- (coh-t.150)
			node[midway,sloped,above] {Traj. reconst.};
		\draw[stealth-,unsure] (coh-xt-2.200) -- (coh-t.30)
			node[midway,sloped,above] {Detector struct.};
		\draw[-stealth] (coh-xt-2.210) -- (coh-t.20)
			node[midway,sloped,below] {Local field resp.};
		\draw[unsure,-stealth] ([xshift=1ex] coh-t.south) -- ([xshift=1ex] field-t.north)
			node[midway,right,align=left] {Field\\ (vacuum +\\ excitations)};
		\draw[stealth-] ([xshift=-1ex] coh-t.south) -- ([xshift=-1ex] field-t.north);
		\draw[-stealth] (field-xt-2.140) -- (field-t.325)
			node[midway,sloped,above] {Local field resp.};
		\draw[stealth-,unsure] (field-xt-2.155) -- (field-t.300)
			node[midway,sloped,below] {Mode decomp.};
		\draw[stealth-,unsure] (field-xt-1.25) -- (field-t.240)
			node[midway,sloped,below] {Mode decomp.};
		\draw[-stealth] (field-xt-1.40) -- (field-t.215)
			node[midway,sloped,above] {Trajectory};
	\end{scope}
\end{tikzpicture}


==> tikz/fourier-quadrants.tex <==
\begin{tikzpicture}[scale=0.5]
\def\str{0.3}
\def\xlen{4.8}
\def\ymax{4.8}
\def\ymin{-4.8}
\tikzstyle{dot}=[draw,circle,minimum size=3pt,inner sep=0pt,
	outer sep=0pt,fill]

\def\fact{0.9}

\def\colabs{blue!30}
\def\colem{purple!35}
\def\colcoh{red!70!orange!35}

\fill[\colabs] (0,0) -- (\fact*\ymax,\fact*\ymax) --
	(-\fact*\ymax,\fact*\ymax) -- cycle;
\fill[\colem] (0,0) -- (-\fact*\ymax,-\fact*\ymax) --
	(\fact*\ymax,-\fact*\ymax) -- cycle;

\draw[->] (0,\fact*1.05*\ymin) -- (0,1.1*\ymax) node[left] {$\omega$};

\node[align=center,fill=\colabs,font=\scriptsize]
at (0,\ymax*0.6) {Absorption\\ processes};
\node[align=center,fill=\colem,font=\scriptsize]
at (0,-\ymax*0.6) {Emission\\ processes};

\fill[\colcoh] (0,0) -- (\fact*\ymax,-\fact*\ymax) --
	(\fact*\xlen,-\fact*\ymax) -- (\fact*\xlen,\fact*\ymax) --
	(\fact*\ymax,\fact*\ymax) -- cycle;
\fill[\colcoh] (0,0) -- (-\fact*\ymax,-\fact*\ymax) --
	(-\fact*\xlen,-\fact*\ymax) -- (-\fact*\xlen,\fact*\ymax) --
	(-\fact*\ymax,\fact*\ymax) -- cycle;
\draw[->] (-\xlen,0) -- (\xlen,0) node[below] {$\frac{\delta\omega}{2}$};

\node[align=center,font=\scriptsize]
at (\xlen*0.48,0) {Abs/Emission\\ coherences};
\node[align=center,font=\scriptsize]
at (-\xlen*0.48,0) {Abs/Emission\\ coherences};

\draw[->] (\ymin,\ymin) -- (\ymax,\ymax)
	node[below right] {$\omega_1$};
\draw[->] (-\ymin,\ymin) -- (-\ymax,\ymax)
	node[below left] {$\omega_2$};

\draw[thick] (\fact*\ymin,\fact*\ymin) -- (\fact*\ymax,\fact*\ymax);
\draw[thick] (-\fact*\ymin,\fact*\ymin) -- (-\fact*\ymax,\fact*\ymax);



\end{tikzpicture}

